Proportionally Fair Matching via Randomized Rounding

Given an edge-colored graph, the goal of the proportional fair matching problem is to find a maximum weight matching while ensuring proportional representation (with respect to the number of edges) of each color. The colors may correspond to demographic groups or other protected traits where we seek to ensure roughly equal representation from each group. It is known that, assuming ETH, it is impossible to approximate the problem with $\ell$ colors in time $2^{o(\ell)} n^{\mathcal{O}(1)}$ (i.e., subexponential in $\ell$) even on \emph{unweighted path graphs}. Further, even determining the existence of a non-empty matching satisfying proportionality is NP-Hard. To overcome this hardness, we relax the stringent proportional fairness constraints to a probabilistic notion. We introduce a notion we call $\delta$-\textsc{ProbablyAlmostFair}, where we ensure proportionality up to a factor of at most $(1 \pm \delta)$ for some small $\delta >0$ with high probability. The violation $\delta$ can be brought arbitrarily close to $0$ for some \emph{good} instances with large values of matching size. We propose and analyze simple and fast algorithms for bipartite graphs that achieve constant-factor approximation guarantees, and return a $\delta$-\textsc{ProbablyAlmostFair} matching.

==> experiments.tex <==
\section{Experiments}
\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{images/plots/objective_bipartite.png}
    \caption[Objective values achieved by fair matching algorithms]{Objective values (i.e., matching weight) achieved by fair matching algorithms. ``Vanilla matching'' shows the objective value of the non-fair LP (without constraints~\eqref{eq:coloring_constraint}). The $x$-axis corresponds to the number of vertices $n$ of the graph, and the $y$-axis to the average matching weight achieved over all instances of size $n$.}
    \label{fig:experiments-objectives}
\end{figure}

We tested our proposal-resolution algorithm (referred to here as~\dglsproposal{}) against the greedy ``peeling'' algorithm of~\citet{bandyapadhyay2023proportionally} (\bgpeeling{}). Our dataset consists of $1440$ randomly generated synthetic graphs. Half of the graphs are $G(n,p)$ Erd\H{o}s-Renyi random graphs with $n \in \{50, 250, 500, 1000 \}$, $p \in \{ \frac{10}{n}, 0.5, \frac{\log^2(n)}{n} \}$, and $\ell \in \{2, 3, \lceil \log(n) \rceil \}$, using $(\alpha, \beta) \in \{ (\frac{.9}{\ell}, \frac{1.1}{\ell}), (\frac{.75}{\ell}, \frac{1.25}{\ell}) \}$; we generated 10 graphs for each combination of these parameters (for a total of $720$).
The other half of the graphs are bipartite graphs generated by sampling a random bipartition in each of the aforementioned graphs (including only the edges crossing the bipartition). 
In all graphs, the edge colors are sampled u.a.r., and edge weights are sampled u.a.r.\ from~$[1,2)$.
The graphs were created in NetworkX~3.1, the algorithms are implemented in Python 3.10.4, and the linear programs are written and solved with Gurobi~10.0.2. 

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{images/plots/priceoffairness.png}
    \caption[Price of Fairness]{The \emph{price of fairness} of the two fair matching algorithms considered, i.e., the ratio between the objective value of the non-fair LP and the weight of the matching achieved by the algorithm.}
    \label{fig:pof}
\end{figure}

% For each graph, we run our algorithm four times, using a slightly different LP each time. For two of the runs, we use the standard LP formulation for bipartite matching (i.e., LP~\eqref{lp:fairmat} without the fairness constraints~\eqref{eq:coloring_constraint}), and for two of the runs, we use the fair LP~\eqref{lp:fairmat}; for each of these, one run uses the randomly generated graph weights and one run treats the graph as \emph{unweighted}. The greedy peeling algorithm of~\citet{bandyapadhyay2023proportionally} does not use LP-based techniques and does not consider edge weights, so we run the algorithm only once on each graph.  
In addition to solving the fair LP, we also solve the standard bipartite matching LP (i.e., LP~\eqref{lp:fairmat} without the fairness constraints~\eqref{eq:coloring_constraint}) on each of our graphs, to determine the maximum non-fair matching as a benchmark against which to compare the results of the fair algorithms. 
% and compare this against the matching produced by the fair algorithms, to assess the impact that introducing fairness has on the size (or weight) of the matching found.

\Cref{fig:experiments-objectives} shows the objective value (i.e., total weight of the matching) found by the two algorithms \bgpeeling{} and \dglsproposal{} as well as the objective value for the non-fair LP. We can see that for bipartite graphs, our algorithm performs extremely well, achieving a matching size close to the optimal non-fair matching. 
% In the case of general graphs, our algorithm achieves a matching of weight about half that of the best non-fair matching. This makes sense, since the sampling of the random bipartite subgraph loses half of the edges in expectation (see~\cref{sec:general-graphs}).
\Cref{fig:pof} shows the \emph{price of fairness}, i.e.\ the ratio between the non-fair LP objective value (shown as ``Vanilla matching'' in~\cref{fig:experiments-objectives}) and the weight of the achieved matching. As expected from the results shown in~\cref{fig:experiments-objectives}, for \dglsproposal{}, this ratio is close to one for bipartite graphs. For \bgpeeling{}, the ratio is much higher, suggesting a much greater loss in matching weight relative to the non-fair optimum. This is not entirely unexpected, since the algorithm greedily attempts to include edges of each color one-for-one, achieving a proportion very close to $1/\ell$ for each color; it is not unexpected that this stricter adherence to proportionality may result in a smaller matching compared to an algorithm that allows the proportion to go be closer to the lower and upper bounds of $\alpha$ and $\beta$, respectively.

Finally, since our algorithm allows for some small violation of the fairness constraints, we are also interested in how large this fairness violation may be. To this end, we compute the factor by which the proportional makeup of any one color in the matching (found by \dglsproposal{}) may be under or over the bounds $\alpha$ and $\beta$, respectively. We do the same for \bgpeeling{}. The results are shown in \cref{fig:fairness-violation}. Unsurprisingly (due to the one-for-one addition of edges for each color, as mentioned in the previous paragraph), \bgpeeling{} did better in this regard than our \dglsproposal{} algorithm, achieving a ratio less than one in some cases (meaning the proportional representation of each color was well within the range of $(\alpha, \beta)$). For \dglsproposal{}, \cref{thm:thm_two_sided_fairness} give theoretical guarantees on how large the violation may be, but
our experimental results suggest that the violation may typically be less than this in practice: it is about $1.2$ at most (when $n$ is small), and becomes close to $1$ for larger $n$.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\columnwidth]{images/plots/fairness_violations.png}
    \caption[Fairness Violations]{Fairness violations. The $y$-axis indicates the violation of the lower or upper bound on the proportionality constraints: for the lower bound, it is the ratio between $\alpha$ (the proportionality lower bound) and the actual proportional composition of the least-represented color, while for the upper bound it is the ratio between the proportional composition of the most-represented color and $\beta$ (the proportionality upper bound)}
    \label{fig:fairness-violation}
\end{figure}

% Plots will include comparisons between the objectives achieved by each algorithm and fairness results. In the case of bipartite graphs, we have access to the optimal matching objectives via the objective of the vanilla LPs and can thus easily report a PoF. We expect i) our algorithm to greatly outperform the greedy peeling algorithm on weighted graphs; ii) our algorithm should perform better on bipartite graphs, as we can skip the initial step of dropping edges.

% Notably, the greedy peeling algorithm took much longer \jl{will look closer, but maybe 8x the amount of time?} as it iterates over all possible optimal objective values between $c$ and $n$. We will make this scaling issue more to emphasize our contribution.

Finally, we also note that \dglsproposal{} was faster in practice, with \bgpeeling{} taking noticeably longer (it took \dglsproposal{} roughly 2 hours total to solve the LPs and compute matchings for all instances combined, while \bgpeeling{} took nearly 2 days to do the same). This is despite the fact that \bgpeeling{} is a simple greedy algorithm while \dglsproposal{} requires solving an LP as an initial step. This difference is likely due to the fact that \bgpeeling{} must iterate over all possible optimal objective values between $\ell$ and $n$; in contrast, the rounding step of \dglsproposal{} is extremely simple, requiring just one random sample per vertex, while the LP~\eqref{lp:fairmat} is a simple LP that we might expect to be solved very quickly by sophisticated LP solvers. 
% \npg{Do we have data we can share here? Any plots, or at least an average running time for some instances or something? Otherwise, reviewers may complain if we make such claims without presenting experimental data to support it.}

% \subsection{General graphs}

% \Cref{TODO} shows the performance comparison between the objectives achieved by \bgpeeling{} and \dglsproposal{}. We see that \bgpeeling{} outperforms

% \subsection{Bipartite graphs}
% % Algorithms : Peeling algorithm, Our algorithm. 
% % Plots : Bandyapadhyay

% \Cref{TODO} shows the performance comparison between objectives achieved by each algorithm, along with results on fairness. The non-fair LP solution allows us to calculate the \emph{price of fairness} of our algorithm (i.e., the ratio between the optimal non-fair matching and the fair matching produced by our proposal algorithm); this price of fairness is plotted in \Cref{TODO}. \npg{Add plots and ref}

% We further note that the peeling algorithm



% \subsection{Fairness violation}

% For all the above algorithms, we would like to compare the multiplicative factor violations in both upper and lowerbounds. 

==> space-tricks.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For Submissions, acmart template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setcopyright{none}
\renewcommand\footnotetextcopyrightpermission[1]{} % This line removes the footnote about the conference and year.
\def\@titlefont{\huge\sffamily\bfseries} % THIS LINE CHANGES THE FONT OF THE TITLE

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% PENALTY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% See their definitions and default values in: https://en.wikibooks.org/wiki/TeX/penalty
\binoppenalty=700
\brokenpenalty=0 %100
\clubpenalty=150   %150
\displaywidowpenalty=50   %50
\exhyphenpenalty=0 %50
\floatingpenalty=0 %20000
\hyphenpenalty=0 %50
\interlinepenalty=0
\linepenalty=10
\postdisplaypenalty=0
\predisplaypenalty=0 %10000
\relpenalty=0 %500
\widowpenalty=0  %150

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Floating: Figure / Table / Algorithm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{float}
\usepackage[labelfont=bf,font={small},aboveskip=0em, belowskip=0em]{caption}

%%%%%%%%%% Floating Spacing %%%%%%%%%%%%%
% Can also set space around the caption separately
%\setlength\abovecaptionskip{0em}
%\setlength\belowcaptionskip{0em}
% Space between multiple floatings
\setlength{\floatsep}{0em}
% space below floating (distance to the rest of text)
\setlength{\textfloatsep}{0.5em}
% space above tables/figures (distance from the text above)
% for tables in the middle of the page (i.e., not top or bottom), this number is both the top spacing and bottom spacing
\setlength{\intextsep}{0.5em}
%%%%% These two are for double-column floatings, e.g., figure* and table*
\setlength{\dbltextfloatsep}{1em} % floating to text
\setlength{\dblfloatsep}{0.5em} % between floatings


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section titles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{titlesec}
%% Change section and subsection title to normal font size
%\titleformat{\section}{\normalfont\large\bfseries}{\thesection}{1em}{}
%\titleformat{\subsection}{\normalfont\large\bfseries}{\thesection}{1em}{}

% Change title spacing
\titlespacing{\section}{0pt}{0.3em}{0.2em} % left margin, space before, space after
\titlespacing{\subsection}{0pt}{0.3em}{0.15em} % left margin, space before, space after
\titlespacing{\subsubsection}{0pt}{0.3em}{0.5em} % left margin, space before, space after (horizontal)
%\newcommand{\mysubsubsection}[1]{\underline{#1}.}
%\titleformat{\subsubsection}[runin]
%{\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{\mysubsubsection}

%\newcommand{\para}[1]{{\bf \emph{#1}}\,}
%\newcommand{\myparagraph}[1]{\noindent\emp{#1} \quad}


